Enriching Ontology with Temporal Commonsense for Low-Resource Audio Tagging

Audio tagging aims at predicting sound events occurred in a recording. Traditional models require enormous laborious annotations, otherwise performance degeneration will be the norm. Therefore, we investigate robust audio tagging models in low-resource scenarios with the enhancement of knowledge graphs. Besides existing ontological knowledge, we further propose a semi-automatic approach that can construct temporal knowledge graphs on diverse domain-specific label sets. Moreover, we leverage a variant of relation-aware graph neural network, D-GCN, to combine the strength of the two knowledge types. Experiments on AudioSet and SONYC urban sound tagging datasets suggest the effectiveness of the introduced temporal knowledge, and the advantage of the combined KGs with D-GCN over single knowledge source.

==> related.tex <==
\section{Related Work}

Traditional audio tagging models are typically based on CNNs \citep{kong2019cross,kong2020panns,gong2021psla}, while the utilization of knowledge is still under-explored. Recently, some works tried to leverage GCNs to model the relationships between labels. \citep{shrivaslava2020mt} proposed to leverage the AudioSet ontology, while \citep{wang2020modeling} constructed co-occurrence graph with the statistics of training data. \citep{sun2020ontology} utilized both co-occurrence graph and the 2-level SONYC ontology. However, this approach requires the mutual prediction of fine/coarse labels, which restricts its application to ontologies with more levels, such as AudioSet. Our method can combine the strength of ontological and temporal knowledge with no need of data statistics, which may not be reliable in low-resource cases, and is generalizable to more domains.

